Graph-based Clustering under Differential Privacy

In this paper, we present the first differentially private clustering method for arbitrary-shaped node clusters in a graph. This algorithm takes as input only an approximate Minimum Spanning Tree (MST) $\mathcal{T}$ released under weight differential privacy constraints from the graph. Then, the underlying nonconvex clustering partition is successfully recovered from cutting optimal cuts on $\mathcal{T}$. As opposed to existing methods, our algorithm is theoretically well-motivated. Experiments support our theoretical findings.

==> DP_background.tex <==
Let us first consider some arbitrary dataset space $\mathcal{D}$, and $``\sim"$ a neighborhood notion on that space (this neighborhood should be understood more as an equivalence relation between two close sets rather than a topological neighborhood).
\begin{definition}[\cite{Dwork_2006}]
A randomized algorithm $\mathcal{A}$ with domain $\mathcal{D}$ is called $(\epsilon,\delta)$-differentially private if for any $S \subset Range(\mathcal{A})$ and for all $x,y \in \mathcal{D}$ such that $x\sim y$, $$\mathbb{P}[\mathcal{A}(x) \in S] \leq e^{\epsilon}\mathbb{P}\left[\mathcal{A}(y) \in S\right] + \delta .$$
Where the probability space is over the coin flips of $\mathcal{A}$.
If $\delta=0$, $\mathcal{A}$ is said to be $\epsilon$-differentially private.
\end{definition}

This formal definition provides a guarantee that under a reasonable choice of privacy degree $\epsilon$, two neighboring datasets produce statistically indistinguishable~\footnote{The notion of statistical indistinguishableness relies on a divergence between statistics. Our work focuses on the neighborhood between databases. We accept without further discussion the common definition using the max-divergence~\cite{Dwork_2013}.} results.
One of the first, and most used differentially private mechanisms is the Laplace mechanism. It is based on the process of releasing a numerical query perturbed by a noise drawn from a centered Laplace distribution scaled to the sensitivity of the query.

\begin{definition}[\cite{Dwork_2006}]
For any $f:\mathcal{D} \rightarrow \mathbb{R}^{k}$, the sensitivity of the function is defined as$$\Delta f=\max\limits_{x\sim y \in \mathcal{D}}||f(x) -f(y)||_{1}.$$ 
\end{definition}

\begin{definition}[\cite{Dwork_2006}]
Given any function $f: \mathcal{D} \rightarrow \mathbb{R}^{k}$,  any $ \epsilon > 0$, and $x\in \mathcal{D}$, the Laplace mechanism is
$$ \mathcal{M}_{L}(x,f,\epsilon)=f(x) + (Y_{1},...,Y_{k})$$
where $Y_{i}$ are i.i.d. random variables drawn from Lap$(\Delta f/\epsilon)$, and Lap$(b)$ denotes the Laplace distribution with scale b $\left(\textit{{\em i.e} probability density }\frac{1}{2b}\exp\left(-\frac{|x|}{b}\right)\right)$.
\end{definition}

\begin{theorem}[\cite{Dwork_2006}]
\label{thm:Laplace}
The Laplace mechanism is $\epsilon$-differentially private.
\end{theorem}

Laplace mechanism is mostly used to answer privately numerical queries, whereas
the Exponential mechanism, represents a way of privately answering arbitrary range queries. Given some range of possible responses to the query $\mathcal{R}$, it is defined according to a utility function $u:= \mathcal{D} \times \mathcal{R} \rightarrow \mathbb{R}$, which aims at providing some total preorder on the range $\mathcal{R}$ according to the total order in $\mathbb{R}$. 
The sensitivity of this function is denoted $\Delta u := \max\limits_{r \in \mathcal{R}} \max\limits_{ x \sim y \in \mathcal{D}} | u(x,r) - u(y,r)|$ .

\begin{definition}[\cite{mechanism-design-via-differential-privacy}]
Given some output range $\mathcal{R} $, some privacy parameter $\epsilon > 0$, some utility function $u:= \mathcal{D} \times \mathcal{R} \rightarrow \mathbb{R}$, and some $x \in \mathcal{D}$, the Exponential mechanism $\mathcal{M}_{Exp}(x, u, \mathcal{R}, \epsilon)$ outputs an element $r \in \mathcal{R}$ with probability proportional to $\exp \left(\frac{\epsilon u(x,r)}{2 \Delta u}\right)$.
\end{definition}

The Exponential mechanism defines a distribution on a potentially complex and large range $\mathcal{R}$. As the following theorem states,  sampling from such a distribution preserves $\epsilon$-differential privacy. 

\begin{theorem}[\cite{mechanism-design-via-differential-privacy}]
\label{th:privacyexpmechanism}
For any non-empty range $\mathcal{R}$, the Exponential mechanism preserves $\epsilon$-differential privacy, \emph{i.e} if $x\sim y \in \mathcal{D}, $ $$\mathbb{P}\left[\mathcal{M}_{Exp}\left(x, u, \mathcal{R}, \epsilon\right) =r\right] \leq e^{\epsilon}\mathbb{P}\left[\mathcal{M}_{Exp}\left(y, u, \mathcal{R}, \epsilon \right) =r\right]. $$
\end{theorem}

Any private mechanism has to make a trade-off between privacy and accuracy. The Exponential mechanism does not constitute an exception to the rule. The following theorem highlights this trade-off for the Exponential mechanism when $ 0< |\mathcal{R}| <  +\infty$.

\begin{theorem}[reformulation \cite{Dwork_2013}]
\label{tradeoffexponential}
Given some dataset $x \in \mathcal{D}$, some output range $\mathcal{R}$, some privacy parameter $\epsilon > 0$, some utility function $u:= \mathcal{D} \times \mathcal{R} \rightarrow \mathbb{R}$, and denoting $OPT_{u}(x)=\max\limits_{r \in \mathcal{R}}u(x,r)$, one has $\forall$ $ t \in \mathbb{R}$, 
$$u\left(x,\mathcal{M}_{Exp}\left(x,u,\mathcal{R},\epsilon \right)\right)\leq OPT_{u}(x) - \frac{2\Delta u}{\epsilon}\left(t + \ln|\mathcal{R}|\right)$$ with probability at most $\exp(-t)$.
\end{theorem}

The main interest of differential privacy is its ability to comply with composition. Let us now introduce this property.

\begin{theorem}[\cite{dwork2006our}] 
\label{thm:basic-composition}
For any $\epsilon >0, \delta \geq 0$ the adaptive composition of $k$ $(\epsilon,\delta)$-differentially private mechanisms is $(k\epsilon,k\delta)$-differentially private.
\end{theorem}

Finally, since it will be useful in the sequel, let us introduce the post-processing property of differential privacy.

\begin{theorem}[Post-Processing~\cite{Dwork_2013}] 
\label{thm:postprocessing}
Let $\mathcal{A}:\mathcal{D} \rightarrow B$ be a randomized algorithm that is $(\epsilon,\delta)$-differentially private,  and $h : B \rightarrow B'$ a deterministic mapping.
Then $h \circ \mathcal{A}$ is $(\epsilon,\delta)$-differentially private.
\end{theorem}
